H2LooP Spark Preview: Continual Pretraining of Large Language Models for Low-Level Embedded Systems Code

Large language models (LLMs) demonstrate strong code generation abilities in general-purpose programming languages but remain limited in specialized domains such as low-level embedded systems programming. This domain involves hardware register manipulation, vendor-specific SDKs, real-time operating system APIs, and hardware abstraction layers that are underrepresented in standard pretraining corpora. We introduce H2LooP Spark Preview, a continual pretraining (CPT) pipeline that adapts the OLMo-3-7B-a fully open language model to the embedded systems domain using BF16 LoRA with rank-stabilized scaling on 8 NVIDIA H100 GPUs. Our training corpus is constructed from repository-datasheet pairs covering 100B tokens of raw embedded systems data across 117 manufacturers, processed using the hierarchical datasheet-to-code mapping approach proposed in SpecMap (Nipane et al., 2026). The resulting curated dataset split contains 23.5B tokens across 13 embedded domains. Continual pretraining with high-rank LoRA (r=512) yields substantial gains, reducing in-domain perplexity by 70.4% and held-out repository perplexity by 66.1%. On generative code completion benchmarks spanning 13 embedded domains, our 7B model outperforms Claude Opus 4.6 and Qwen3-Coder-30B on 8 categories in token accuracy, showing that targeted continual pretraining enables smaller open-weight models to rival frontier systems on specialized technical tasks. We release the production training checkpoint on Huggingface as an open-source artifact.

==> sections/references.tex <==
\begin{thebibliography}{99}

\bibitem{biderman2024lora}
Biderman, S., et al. (2024). LoRA Learns Less and Forgets Less. \textit{TMLR}.

\bibitem{bolton2024biomedlm}
Bolton, E., et al. (2024). BioMedLM: A 2.7B Parameter Language Model Trained On Biomedical Text. \textit{Nature}.

\bibitem{chen2021codex}
Chen, M., et al. (2021). Evaluating Large Language Models Trained on Code. \textit{arXiv:2107.03374}.

\bibitem{colombo2024saullm}
Colombo, P., et al. (2024). SaulLM-7B: A Pioneering Large Language Model for Law. \textit{arXiv:2403.03883}.

\bibitem{dao2023flashattention2}
Dao, T. (2023). FlashAttention-2: Faster Attention with Better Parallelism and Work Partitioning. \textit{ICLR}.

\bibitem{dettmers2023qlora}
Dettmers, T., et al. (2023). QLoRA: Efficient Finetuning of Quantized Language Models. \textit{NeurIPS}.

\bibitem{feng2020codebert}
Feng, Z., et al. (2020). CodeBERT: A Pre-Trained Model for Programming and Natural Languages. \textit{EMNLP}.

\bibitem{groeneveld2024olmo}
Groeneveld, D., et al. (2024). OLMo: Accelerating the Science of Language Models. \textit{ACL}.

\bibitem{teamolmo2025olmo3}
Team OLMo (2025). OLMo 3. \textit{arXiv:2512.13961}.

\bibitem{gupta2023continual}
Gupta, K., et al. (2023). Continual Pre-Training of Large Language Models: How to (re)warm your model? \textit{arXiv:2308.04014}.

\bibitem{guo2021graphcodebert}
Guo, D., et al. (2021). GraphCodeBERT: Pre-training Code Representations with Data Flow. \textit{ICLR}.

\bibitem{guo2024deepseek}
Guo, D., et al. (2024). DeepSeek-Coder: When the Large Language Model Meets Programming. \textit{arXiv:2401.14196}.

\bibitem{hu2022lora}
Hu, E.J., et al. (2022). LoRA: Low-Rank Adaptation of Large Language Models. \textit{ICLR}.

\bibitem{hui2024qwen}
Hui, B., et al. (2024). Qwen2.5-Coder Technical Report. \textit{arXiv:2409.12186}.

\bibitem{kalajdzievski2023rslora}
Kalajdzievski, D. (2023). Scaling Up: A Review of Normalized Initialization for Low-Rank Adaptation. \textit{arXiv:2312.03732}.

\bibitem{li2023starcoder}
Li, R., et al. (2023). StarCoder: May the Source Be With You. \textit{TMLR}.

\bibitem{liu2024chipnemo}
Liu, M., et al. (2024). ChipNeMo: Domain-Adapted LLMs for Chip Design. \textit{DAC}.

\bibitem{nipane2026specmap}
Nipane, V., Agrawal, P., and Singh, A. (2026). SpecMap: Hierarchical LLM Agent for Datasheet-to-Code Traceability Link Recovery in Systems Engineering. \textit{arXiv:2601.11688}.

\bibitem{robertson2009bm25}
Robertson, S., and Zaragoza, H. (2009). The Probabilistic Relevance Framework: BM25 and Beyond. \textit{FnTIR}.

\bibitem{roziere2023codellama}
Roziere, B., et al. (2023). Code Llama: Open Foundation Models for Code. \textit{arXiv:2308.12950}.

\bibitem{singh2025convergence}
Singh, A., Nipane, V., and Agrawal, P. (2025). On Convergence Dynamics in Fine-Tuning Strategies for Large Language Models. H2LooP.ai Blog. \url{https://www.h2loop.ai/resources/blog/on-convergence-dynamics-in-fine-tuning-strategies-for-large-language-models}.

\bibitem{wang2024traceability}
Wang, J., et al. (2024). Traceability Link Recovery: How Far Are We? \textit{arXiv:2509.05585}.

\end{thebibliography}

